Text Summarization with Latent Queries

The availability of large-scale datasets has driven the development of neural models that create summaries from single documents, for generic purposes. When using a summarization system, users often have specific intents with various language realizations, which, depending on the information need, can range from a single keyword to a long narrative composed of multiple questions. Existing summarization systems, however, often either fail to support or act robustly on this query focused summarization task. We introduce LaQSum, the first unified text summarization system that learns Latent Queries from documents for abstractive summarization with any existing query forms. Under a deep generative framework, our system jointly optimizes a latent query model and a conditional language model, allowing users to plug-and-play queries of any type at test time. Despite learning from only generic summarization data and requiring no further optimization for downstream summarization tasks, our system robustly outperforms strong comparison systems across summarization benchmarks with different query types, document settings, and target domains.

==> tab_ablation.tex <==
%% All data for Ablation Study
\begin{table*}[t]
\footnotesize
\tabcolsep=0.07cm
\bgroup
\def\arraystretch{1.0}
\centerline{
% \begin{small}
% \begin{tabular}{@{}l@{~}@{~}c@{~~}c@{~~}cc@{~~}c@{~~}c@{}}  % The first row
\begin{tabular}{lccc ccc ccc ccc ccc ccc}
\hline
\multirow{1}*{\textbf{Models}} 
& \multicolumn{3}{c}{\textbf{CNN/DM}}
& \multicolumn{3}{c}{\textbf{WikiRef}}
& \multicolumn{3}{c}{\textbf{Debatepedia}}
& \multicolumn{3}{c}{\textbf{DUC 2006}}
& \multicolumn{3}{c}{\textbf{DUC 2007}}
& \multicolumn{3}{c}{\textbf{TD-QFS}}\\
~ & {R-1} & {R-2} & {R-L} 
& {R-1} & {R-2} & {R-L} 
& {R-1} & {R-2} & {R-L}
& {R-1} & {R-2} & {R-SU4} 
& {R-1} & {R-2} & {R-SU4} 
& {R-1} & {R-2} & {R-SU4}
\\
\hline
{\textsc{LaQSum}}
& {45.1}	& {22.0}	& {41.9}
& {31.1}	& {12.6}	&{27.1}
& {23.5}	&\hspace{0.5em}{7.2}    &{20.6}
&{39.1}	&\hspace{0.5em}{8.5}	&{13.7	}
&{40.4}	&{10.2}	&{15.0}
&{45.7}	&{18.1}	&{22.1}
\\
{\hspace*{2ex}-$\Delta(\hat{\mathbf{z}}|\mathbf{x},\mathbf{z})$}
& --- & --- & --- 
&$\downarrow$0.1 &$\downarrow$0.2 &$\downarrow$0.2
&$\downarrow$0.5 &$\downarrow$0.3 &$\downarrow$0.6
&$\downarrow$0.6	
&$\downarrow$0.2	
&$\downarrow$0.6	
&$\uparrow$0.1	
&$\downarrow$0.1	
&$\downarrow$1.3
&$\uparrow$0.1	
&$\downarrow$0.6	
&$\downarrow$0.4
\\
{\hspace*{2ex}-Joint training}
&$\downarrow$0.4	&$\downarrow$0.3	&$\downarrow$0.4	&$\downarrow$2.9	&$\downarrow$0.9	&$\downarrow$2.8
&$\downarrow$2.8	&$\downarrow$1.1	&$\downarrow$2.8	
&$\downarrow$2.9	&$\downarrow$1.7	&$\downarrow$1.6	
&$\downarrow$2.4	&$\downarrow$2.0	&$\downarrow$1.7
&$\downarrow$0.7	
&$\downarrow$0.6	
&$\downarrow$0.4
\\
{\hspace*{2ex}-Weak supervision}
&$\downarrow$0.6	&$\downarrow$0.7	&$\downarrow$0.7	
&$\downarrow$0.7	&$\downarrow$0.2	&$\downarrow$0.5	
&$\downarrow$1.0	&$\downarrow$0.5	&$\downarrow$1.3
&$\downarrow$0.2	&$\downarrow$0.2	&$\downarrow$0.2	
&$\downarrow$0.2	&$\downarrow$0.3	&$\downarrow$0.3
&$\downarrow$0.1	&$\downarrow$0.3	&$\downarrow$0.0
\\
{\hspace*{2ex}-Dual view}
&$\downarrow$2.7	
&$\downarrow$3.5	
&$\downarrow$2.5
&\hspace{0.5em}$\downarrow$12.2	&$\downarrow$9.3	&$\hspace{0.5em}\downarrow$10.5	
&$\downarrow$7.9	&$\downarrow$3.3	&$\downarrow$6.6	
&$\downarrow$6.3	&$\downarrow$1.8	&$\downarrow$1.8	
&$\downarrow$6.5	&$\downarrow$3.0	&$\downarrow$2.5	
&$\downarrow$2.5	&$\downarrow$3.3	&$\downarrow$2.8
\\
{\hspace*{2ex}-Posterior dropout}
&$\downarrow$0.7	&$\downarrow$0.6	&$\downarrow$0.8	
&$\downarrow$0.8	&$\downarrow$0.3	&$\downarrow$0.7
&$\downarrow$1.1	&$\downarrow$0.3	&$\downarrow$1.2	
&$\downarrow$0.2	&$\downarrow$0.2	&$\downarrow$0.2	
&$\downarrow$0.4	&$\downarrow$0.4	&$\downarrow$0.5
&$\uparrow$0.2	
&$\downarrow$0.0	
&$\uparrow$0.1
\\
\hline
\end{tabular}
% \end{small}
}
\egroup
\caption{\label{tab:ablation} 
  Ablation results for our abstractive summarization system.
}
\end{table*}

==> tab_main.tex <==
\begin{table*}[t]
% \footnotesize
% \tabcolsep=0.1cm
\bgroup
% \def\arraystretch{1.0}
\centerline{
% \begin{small}
\begin{tabular}{lccc ccc ccc}
\hline
\multirow{2}*{\textbf{Systems}} 
& \multicolumn{3}{c}{\textbf{CNN/DM}} 
& \multicolumn{3}{c}{\textbf{WikiRef}}
& \multicolumn{3}{c}{\textbf{Debatepedia}}\\
~ & {R-1} & {R-2} & {R-L} 
& {R-1} & {R-2} & {R-L} 
& {R-1} & {R-2} & {R-L} \\
\thickhline
{\sc Oracle}
&55.8 &33.2 &51.8 
&54.5 &37.5 &48.5
\\
{\sc Lead}
&40.4	&17.6	&36.7
&26.3 &10.5 &21.8
\\
{\sc BertExt}
&43.9 &20.3 &39.9
% &36.0 &18.8 &30.7
\\
{\sc MatchSum}
&43.9	&20.6	&39.8
\\
\hline
{\sc PointerGenerator}
&39.5 &17.3 &36.4
\\
{\sc BottumUp}
&41.2 &18.7 &38.4
\\
{\sc BertAbs}
&41.7 &19.4 &38.8
\\
{\sc Bart}
&44.2   &21.3   &40.9
&30.0	&12.2	&26.0
\\
{\sc GSum$^\ast$}
&45.9	&22.3	&42.5
\\
{\sc GSum} (ours)
& 45.0	& 21.9	& 41.8
\\
\hline
{\sc  Lacus}
& 45.0	& 21.9	& 41.7
\\
\thickhline
\end{tabular}
}
\egroup
\caption{\label{tab:rank} 
  Supervised performance on CNN/DM and zero-shot performance on WikiRef (with keywords as queries), and Debatepedia (with questions as queries).
  R-1, R-2 and R-L stand for the F1 score of ROUGE~1, 2, and L, respectively. \textsc{GSum} (ours) uses the same configurations (i.e., dataset and optimization) as our model.
}
\end{table*}
